Soundly Handling Linearity

We propose a novel approach to soundly combining linear types with effect handlers. Linear type systems statically ensure that resources such as file handles are used exactly once. Effect handlers provide a modular programming abstraction for implementing features ranging from exceptions to concurrency. Whereas linear type systems bake in the assumption that continuations are invoked exactly once, effect handlers allow continuations to be discarded or invoked more than once. This mismatch leads to soundness bugs in existing systems such as the programming language Links, which combines linearity (for session types) with effect handlers. We introduce control flow linearity as a means to ensure that continuations are used in accordance with the linearity of any resources they capture, ruling out such soundness bugs. We formalise control flow linearity in a System F-style core calculus Feffpop equipped with linear types, effect types, and effect handlers. We define a linearity-aware semantics to formally prove that Feffpop preserves the integrity of linear values in the sense that no linear value is discarded or duplicated. In order to show that control flow linearity can be made practical, we adapt Links based on the design of Feffpop, in doing so fixing a long-standing soundness bug. Finally, to better expose the potential of control flow linearity, we define an ML-style core calculus Qeffpop, based on qualified types, which requires no programmer provided annotations, and instead relies entirely on type inference to infer control flow linearity. Both linearity and effects are captured by qualified types. Qeffpop overcomes a number of practical limitations of Feffpop, supporting abstraction over linearity, linearity dependencies between type variables, and a much more fine-grained notion of control flow linearity.

==> Makefile <==
LATEXMK := $(shell command -v latexmk 2> /dev/null)

TEXC=pdflatex
CFLAGS=-interaction=nonstopmode -halt-on-error -file-line-error
BIBC=bibtex
PAPER=linear-handler
BIBLIO=reference

# Sam wants to use latexmk -- I don't. You can opt out of using
# latexmk by adding your username to the array OPT_OUT below.
BUILD_METHOD=$(PAPER).pdf
OPT_OUT := dhil

all:
  ifndef LATEXMK
    BUILD_METHOD=$(PAPER).pdf
  else
    ifneq ($(filter $(USER),$(OPT_OUT)),)
      BUILD_METHOD=$(PAPER).pdf
    else
      BUILD_METHOD=$(PAPER).pdf-via-latexmk
    endif
  endif
all: $(BUILD_METHOD)

extended: $(BUILD_METHOD)-extended
arxiv: $(BUILD_METHOD)-arxiv
camera-ready: all


crop: $(PAPER).pdf
	pdftk $(PAPER).pdf cat 1-29 output submission.pdf

$(PAPER).aux: $(PAPER).tex
	$(TEXC) $(CFLAGS) $(PAPER)

$(BIBLIO).bbl: $(PAPER).aux $(BIBLIO).bib
	$(BIBC) $(PAPER)

$(PAPER).pdf-arxiv: CFLAGS:=$(CFLAGS) "\def\ARXIV{}\input{$(PAPER)}"
$(PAPER).pdf-arxiv: all

$(PAPER).pdf-extended: CFLAGS:=$(CFLAGS) "\def\EXTENDED{}\input{$(PAPER)}"
$(PAPER).pdf-extended: all

$(PAPER).pdf: $(PAPER).aux $(BIBLIO).bbl
	$(TEXC) $(CFLAGS) $(PAPER)
	$(TEXC) $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk: $(PAPER).tex
	latexmk -pdf $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk-extended: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\EXTENDED{}\input{%S}"' $(PAPER)

$(PAPER).pdf-via-latexmk-arxiv: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\ARXIV{}\input{%S}"' $(PAPER)

clean:
	rm -f *.log *.aux *.toc *.out
	rm -f *.bbl *.blg *.fls *.xml
	rm -f *.fdb_latexmk *.vtc *.cut
	rm -f $(PAPER).pdf camera-ready.pdf submission.pdf
	rm -f *.o *.cmx *.cmo

